On the resilience of cellular networks: how can national roaming help?

Cellular networks have become one of the critical infrastructures, as many services depend increasingly on wireless connectivity. Therefore, it is important to quantify the resilience of existing cellular network infrastructures against potential risks, ranging from natural disasters to security attacks, that might occur with a low probability but can lead to severe disruption of the services. In this paper, we combine models with public data from national bodies on mobile network operator (MNO) infrastructures, population distribution, and urbanity level to assess the coverage and capacity of a cellular network at a country scale. Our analysis offers insights on the potential weak points that need improvement to ensure a low fraction of disconnected population (FDP) and high fraction of satisfied population (FSP). As a resilience improvement approach, we investigate in which regions and to what extent each MNO can benefit from infrastructure sharing or national roaming, i.e., all MNOs act as a single national operator. As our case study, we focus on Dutch cellular infrastructure and model risks as random failures, correlated failures in a geographic region, and abrupt increase in the number of users. Our analysis shows that there is a wide performance difference across MNOs and geographic regions in terms of FDP and FSP. However, national roaming consistently offers significant benefits, e.g., up to 13% improvement in FDP and up to 55% in FSP when the networks function without any failures.

==> 1.introduction.tex <==
\section{Introduction}\label{sec:introduction}

% Discuss why this analysis
% Discuss why mmWave
% Introduce the research questions
% Discuss the contributions: compare-contrast with the literature if any
% Introduce the methodology
% Highlight the key take-aways
%As many measurement studies and report show, 


Cellular networks play a key role in today's communications, as many services depend on the proper functioning of these infrastructures.    
However, they can be vulnerable to failures resulting from various sources such as 
large-scale natural disasters including earthquakes~\cite{mayer-eq-pam21} and wildfires~\cite{anderson-wildfires-imc2020}, cyberattacks on the network infrastructure~\cite{vodafoneportugal, mukherjee2014network}, or regional power shortages~\cite{reutersnews}. 
{These events will either affect certain regions, such as earthquake areas \cite{mayer-eq-pam21}, or can be randomly spread~(e.g., hardware-related failures).}
%
% Moreover, networks can be under stress due to a sudden increase of the number of connected users and bandwidth-hungry applications, e.g., during crowded events~\cite{shafiq2013first}. Under these failures or events, we will analyse whether it is possible to still maintain an acceptable level of service.  
%
% Large-scale disasters such as hurricanes are rare, but often lead to permanent failures of the network infrastructure. Other disruptions, such as weather disruptions, may last shorter, but appear more often, and more importantly, correlated over time. For these types of failures, it is important to take these event location correlations into account, for example by using spatial point processes~\cite{rahnamay2011modeling}. 
% A particular feature of these failures is that they are correlated with the geographical area on which the cellular network functions. Failure events are often more likely to occur in one geographic area than in another, and they often occur in close by locations jointly.
% While these failure-inducing events may not happen on a daily basis, however, once they occur, they might lead to severe disruptions due to the dependency of the critical services on these  infrastructures. }
%
Indeed, the functioning of cellular networks becomes even more important during such failure events, e.g., for rescue and recovery in the aftermath of disasters. The key question then is: \textit{what is the coverage and capacity that a mobile network operator~(MNO) can provide, given some links or network nodes do not function?}%  {\color{brown} Should we also mention something about the disconnected people? I feel that in some cases the QoS might not be the main concern, e.g., sending a simple text message might only require a connection.}
%



% In this paper, we focus on millimetre wave frequencies (mmWave) as operation at higher frequencies is considered by many as a remedy for drastic increase in demand for wireless capacity. 
%
% While these bands offer abundant bandwidth compared to sub-6GHz bands, unfortunately, they are more prone to failures due to weather-induced conditions such as rainfall or fog than lower frequency bands. 
%
% Moreover, blockages might hinder communication capacity significantly. 
%
% In contrast to large-scale disasters such as hurricanes, these weather-induced conditions occur more frequently, and could therefore potentially have a disrupting effect on the 5G network. We here investigate the extent to which such failures can cause a decrease in network performance in terms of its quality of service. 

% A second question that is important in resilience analysis is how the resilience of a given network can be improved. 
While the resilience literature is broad in other areas of critical infrastructures, to the best of our knowledge, there are only few studies on quantifying a cellular network's resilience at a national scale such as \cite{griffith2015measuring} and \cite{yanPredictiveImpact}, the former defining resilience as ``the maximum number of sites that can fail before the performance metric of interest falls below a minimum acceptable threshold", and the latter using the number of served users as the resilience metric. 
% 
Since both ensuring coverage
%\footnote{\newInfo{With coverage we mean users covered by BSs for data connectivity.}}
and satisfying quality of service~(QoS) are important, we use \textit{fraction of disconnected population}~(FDP) and \textit{fraction of satisfied population}~(FSP) \newInfo{considering data services} to quantify the resilience of an MNO. 
%\textcolor{blue}{Can we really say that we introduce these measures? I guess that fraction disconnected has been studied before?}
%
%Using these metrics, we analyze the resilience of the Dutch MNOs, 
%develop strategies to achieve the desired resilience level. While there could be various strategies toward this goal, our focus will mainly be on the use of \textit{multi-connectivity}~(MC). {\color{red}{Is it still the case?}}
% Under MC, a user is simultaneously connected to a network through multiple connections, e.g., base stations~(BS). As the traffic can flow through multiple paths, MC can increase the resilience of a network by exploiting spatial or/and frequency diversity. For instance, a user can be connected to a millimeter wave~(mmWave) network which provides an ample bandwidth while a second link at sub-6GHz bands ensures a stable connection if the mmWave link fails. Regarding spatial diversity, a user can be connected to multiple BSs at different locations, increasing the robustness against network failures.
%
% Another option to improve resilience is to add more capacity, e.g., deployment of new BSs. This introduces extra capacity to the network, that may not be needed during regular service, but that can improve its performance under failures drastically. 
% As a case study, we will focus on the Dutch cellular network,
Combining cell tower data with population density statistics as well as urbanity levels in the Netherlands, we investigate the current state of the Dutch MNOs\footnote{Our analysis can be extended to other countries by providing the data presented in Sec.\ref{sec:data} on the MNO infrastructures, cities, urbanity of each region, and population data of the corresponding countries.} and then study their resilience to (i) random failures which could occur due to human errors and (ii) failures confined to a certain geographical region occurring due to disasters. %, and (iii) a sudden increase in the number of users. %We show that XXX.
The insights from our analysis can help to improve the MNO infrastructures to absorb crises or to recover quickly from their effects. 


While there are various ways to improve the resilience of a cellular network, one approach is \textit{national roaming} which facilitates MNOs to use the infrastructure of each other when needed, e.g., in case its own infrastructure is not functional or does not suffice to serve with the required service levels. 
{For increasing \newInfo{data} coverage, national roaming has already been widely adopted in countries such as India~\cite{indiaRoaming13} where MNOs often operate in certain parts of the country or where infrastructure is not as ubiquitous. In 2022, the Federal Communications Commission (FCC) in the US has introduced \textit{roaming under disasters}~(RuD) based on bilateral agreements between MNOs that requires MNOs to serve each other's users in case of service disruptions due to the infrastructure damage during disasters and emergencies~\cite{fcc2022}. Moreover, in 2022 after national infrastructures are damaged considerably due to the Russian invasion, MNOs in Ukraine implemented national roaming~\cite{ukraineNR2022}.} 
Prior studies such as \cite{ENISA2010} advocate national roaming for more resilient cellular infrastructures, and studies such as \cite{panchal2013mobile} investigate different modes of MNO network sharing. \textit{However, to the best of our knowledge, there is no study quantifying the gains in coverage, capacity, and resilience facilitated by national roaming.}  
% 
Toward filling this gap, we quantify in this paper the gains when MNOs work together to serve all the citizens as a single national operator. 
{Furthermore, to provide some insights to the MNOs or to the national telecommunication regulatory bodies on in which areas and which technologies they could prioritize such roaming agreements, we analyze implementation of roaming in a more restricted way such as in only urban areas or rural areas, or considering a certain technology such as 4G or 5G.} 


To summarize, our goal in this paper is to address the following questions: 
\begin{itemize}
%\item Which metrics can measure the resilience of a cellular network?
\item What is current coverage and capacity of MNOs in the Netherlands? Are there regional differences~(e.g, across cities) or differences among the MNOs? 
%    \item {\color{red}Given a target resilience metric, how can a network operator achieve the desired resilience under a budget constraint, e.g., number of BSs to deploy?}
%\item \textcolor{red}{How does the weather-related disruptions, e.g., rain, wind, and humidity, affect the resilience of a cellular network?}
\item What would be the performance gain if all MNOs act as a single national operator and in which regions will this provide the highest gains? 
\item How resilient are MNOs to various types of failures and how much can national roaming help to ensure resilience of the MNOs against failures?
\item 
%\newInfo{How should national roaming be managed to give the highest benefits in terms of coverage and user satisfaction?}  
{Which technologies (3G, 4G, 5G) or which areas (urban vs. rural) should MNOs consider first implementing such roaming agreements for ensuring the highest benefits in terms of coverage and user satisfaction}  \newInfo{for data services?}


%\item Which BSs will result in the highest decrease in performance in terms of disconnected population or satisfied population when they fail (e.g., individually due to a technical problem or loss of power)? 
%    \item How can multi-connectivity improve the resilience of a cellular network given the impact of weather-related disruptions?
%    \item How does the backhaul connectivity affect the resilience, e.g., microwave vs. mmWave backhauls?
    
\end{itemize}
%While addressing these questions,
In a nutshell, our contributions are as follows:
\begin{itemize}
   \item We provide an approach to assess the resilience of a cellular network using  public data and models on coverage and capacity. To reflect the effect of disruptions on the citizens, we use FDP and FSP as our metrics.  
   \item Using publicly-available data from national bodies in the Netherlands, we assess the current state of the Dutch cellular networks on both province and municipality level.
   \item We show that national roaming leads to significant benefits {in some regions} for both FSP and FDP while there is a large performance difference across MNOs and geographic regions. {These areas with high performance gains from national roaming could be considered first by  MNOs to enter such roaming agreements. Moreover, we provide an analysis of roaming implemented only for certain cellular technologies, e.g., 3G and 5G, and in urban vs. rural areas %to show the potential improvement in coverage and capacity for the MNOs 
   in case MNOs prefer national roaming in a more limited way rather than sharing their all network infrastructures.}
   \item We model two risk scenarios to investigate the resilience of the Dutch MNOs with and without national roaming. Our analysis suggests that MNOs are resilient against isolated failures owing to high \newInfo{base station~(BS)} density. That is, FDP  remains roughly the same. On the contrary, FSP  decreases due to the increased number of users served by the surviving BSs. Meanwhile, the impact of correlated failures is more drastic due to BSs  in the same region becoming dysfunctional simultaneously. {To ensure resilience in such cases, alternative approaches are paramount, e.g., aerial connectivity or cells on wheels.}
   \end{itemize}

The rest of the paper is organized as follows. First, Section~\ref{sec:related} provides an overview of the related work on resilience metrics and analysis of communication networks and national roaming. Then, Section~\ref{sec:system_model} introduces the considered system model which is followed by Section~\ref{sec:res_metrics} that presents the definition of the metrics used in our analysis. Next, Section~\ref{sec:perfeval} presents a case study of Dutch cellular networks\footnote{\newInfo{We share the code and data publicly under  \url{https://github.com/lweedage/disaster-resilience}. }} and publicly-available data, i.e., on MNOs, population statistics, and urbanity levels of different areas. 
Section~\ref{sec:perf-failures} also considers the failures and how they will affect the MNOs. Finally, Section~\ref{sec:discussion} discusses the limitations of our work and Section~\ref{sec:conclusion} draws  conclusions.


==> 2.related.tex <==
\section{Related Work}\label{sec:related}
This section discusses the related work on  \textit{resilience metrics and analysis} and   \textit{national roaming/infrastructure sharing}.
%\textcolor{red}{This section might need rewriting.}\textcolor{purple}{Indeed, maybe we should also add something about redundancy? (National roaming is I guess one way to provide redundancy?)}

\smallskip
\noindent \textbf{Resilience metrics and analysis:} The resilience of networks have been investigated in different contexts, such as in traffic networks~\cite{ganin2017}, power grids~\cite{kim2017network}, ecological networks~\cite{kharrazi2016evaluating} and supply chain networks~\cite{zhao2011analyzing}. %In all these applications, 
The resilience of the network has several aspects: whether the network is operational, and whether the service it offers is acceptable. To represent this distinction, metrics are categorized into two as \textit{topological} and \textit{functional metrics}~\cite{rak2020guide}. Topological metrics, %subdivided into \textit{centrality} and \textit{structural} metrics, 
represent the status of the underlying network's connectivity and network paths, e.g., %Some examples include 
relative size of the largest connected component, average two terminal reliability, average path length, motifs~\cite{dey2019} and spectral metrics~\cite{alenazi2015evaluation}. 
%
While these topological metrics provide useful insights about the existing/surviving infrastructure, they fall short of assessing the satisfaction of the served users and applications. As a remedy, functional metrics including objective~(e.g., link stress and node load~\cite{rak2020guide}) and subjective metrics~(e.g., mean-opinion-score or other quality-of-experience metrics~\cite{natalino2020functional}) aim at assessing to what extent the network can satisfy its users' expectations. 
%These metrics include objective metrics and subjective metrics. Objective metrics quantify the quality of performance at a packet or service level by recording for instance packet loss ratio, average delay and jitter, and throughput. 
%Network level objective metrics include link stress, link utilization, node and link load~\cite{rak2020guide}. 
%Subjective metrics such as  mean-opinion-score (MOS) or other quality-of-experience~(QoE) metrics~\cite{natalino2020functional}, as the name suggests, depend on the users' perception and therefore are difficult to acquire in near-real-time at scale. %These metrics include mean-opinion-score (MOS) or other quality-of-experience~(QoE) metrics~\cite{natalino2020functional}. 
Note that functional metrics need to reflect the application's requirements, e.g., a reliability requiring application will be assessed by packet loss ratio. Some studies focus on static metrics, e.g., performance after the disruptive event, while others measure the system performance over a period of time~\cite{sun2020resilience, lin2020}. Similar to \cite{liang2023holistic}, our study focuses on static resilience using functional metrics, where we investigate the loss in quality of service immediately after a disruptive event.   
% \suzan{This might also be good to mention \cite{liang2023holistic.}} 

When it comes to analyzing the resilience of a network, the closest studies to ours are \cite{griffith2015measuring, yanPredictiveImpact}. Yan et al.\cite{yanPredictiveImpact} propose the metric Tower Outage Impact Predictor~(TOIP) to quantify the impact of a failure of a cell tower on the number of served cellular users. Due to the dense deployment of cell towers, a user might not perceive the failure of a cell-tower as it will be served immediately by another BS in the proximity.  
%
Using the data from an operational MNO, the authors propose a prediction scheme to estimate the number of users who would be affected by service outages of one or more BSs in the network. Our work differs from \cite{yanPredictiveImpact} in that we combine cellular network coverage and capacity models with the real-world data on the cellular network infrastructure to quantify the impact of failures on the user's connectivity and satisfaction performance. Moreover, our focus is also on the potential resilience improvement due to infrastructure sharing among MNOs in the same country. %Our work can be considered as complimentary as 
\textcolor{black}{Contrary to~\cite{griffith2015measuring}, our work investigates both coverage as service quality as metrics, and combines models with several data sources to assess resilience.} 

%Often, a distinction is made between structural and operational resilience~\cite{mauthe2016disaster,alderson2014assessing}. From a structural perspective, resilient networks have redundancy and diversity to enable alternative routes for network traffic. From an operational perspective, networks should be able to detect failures, and respond quickly to make sure that its services recover quickly.
%\lotte{Maybe remove this part and line 26?}
%Other prior works have also investigated resilience of cellular networks against various risks: wildfires~\cite{anderson-wildfires-imc2020}, earthquakes~\cite{mayer-eq-pam21}, and rain~\cite{padmanabhan2019residential}. Wildfires, emerging more frequently with the climate change, might threaten the functioning of the cellular networks as studied in \cite{anderson-wildfires-imc2020} which provides a vulnerability analysis of cellular network infrastructure in the US using the historical wildfire records, wildfire risk projections, and cellular infrastructure deployment. The key conclusion of \cite{anderson-wildfires-imc2020} is that the primary risk is due to possible power outage caused by the wildfires rather than the damage to the network equipment. 
%Furthermore, extremely dense deployment of 5G BSs makes them more vulnerable to changes in their power supply, as this increases the difference between peaks and lows in their traffic demands~\cite{cinkler2020resilience}. 
Authors of \cite{smallcells} consider two kinds of failures that might affect small cells in the Netherlands: power outages and cyberattacks. They investigate a case of power outage in 2015 in Noord-Holland, where after two hours $80\%$ of the BS sites were down. In this case, providers immediately shut down the LTE network to have sufficient power supply for the essential network. Study in \cite{smallcells} proposes to also first deactivate small cells for keeping the emergency services functioning longer.
% Moreover, small cells usually will have no batteries.
%  Small cells might be more susceptible to cyberattacks and be affected more drastically compared to macrocells, as they might have a wireless backhaul to macrocells, which makes it easier to attack multiple cells at once.

% \lotte{Maybe remove this paragraph as this is more about fibre cables?}
% A case study on the Virgin Islands~\cite{wine2020analyzing} identifies areas that are particularly vulnerable to disaster-related failures based on terrain analysis and a path loss model. \cite{mayer-eq-pam21} studies the resilience of the Internet against earthquakes in the Pacific Northwest. The authors show that a non-negligible fraction of the fibre networks and cellular towers are susceptible to earthquake shaking. By identifying the regions where the level of peak ground acceleration is lower, the authors point out to alternate routes for fibre optic cable deployment that require longer cables but increase resilience to earthquake-shaking. 

% 
The resilience of 5G networks is of particular importance, since higher frequencies~(e.g., mmWave  bands) are more prone to errors~\cite{Esposito2018} and links operating at these high bands might be affected by rain drastically, as the rain drops are non-negligible in their size in relation to the wavelength of the mmWave signals~\cite{cinkler2020resilience,hemadeh2017millimeter}. An eight-year measurement study \cite{padmanabhan2019residential} shows that rain might result in internet outages in some regions, and especially wireless links are more prone to these outages.  
\textcolor{black}{Our study differs from these studies in that we combine models and publicly-available data to offer insights on the coverage and capacity performance of MNOs under two failure categories and the potential of national roaming toward mitigating the impact of these failures.}

% \smallskip
% \noindent \textbf{Failure models:} \textcolor{blue}{SB: since related work is too long, maybe remove this failures part and cite some references in Introduction where we talk about two types of failures.}
%We are also interested in the resilience of the network under failures, in particular \textit{disaster-induced} multiple failures \cite{rak2020guide}.
% A communication network might experience failures in its components due to various reasons such as natural disasters, weather-induced disruptions, technology-related failures or malicious attacks~\cite{mukherjee2014network}. These events will either affect certain regions, such as earthquake areas \cite{mayer-eq-pam21}, or can be randomly spread (e.g., technology-related failures).
% %
% Moreover, networks can be under stress due to a sudden increase of the number of connected users and bandwidth-hungry applications, e.g., during crowded events~\cite{shafiq2013first}.  Under these failures or events, we will analyse whether it is possible to still maintain an acceptable level of service.  

% Most disasters only impact a specific geographic area. Therefore, they affect the performance of several nearby network links in a correlated manner.
% %
% For this reason, disasters are often modelled by a geographic area that moves across the network. Links within or close by the disaster area fail with some probability. In such probabilistic geographical failure models, the failure probability usually decreases with the distance to the epicentre of the disaster~\cite{agarwal2013resilience}. 
% Large-scale disasters such as hurricanes are rare, but often lead to permanent failures of the network infrastructure. Other disruptions, such as weather disruptions, may last shorter, but appear more often, and more importantly, correlated over time. For these types of failures, it is important to take these event location correlations into account, for example by using spatial point processes~\cite{rahnamay2011modeling}. 

\smallskip

\textbf{National roaming/infrastructure sharing: }
As resilience can be improved by increasing redundancy and over-provisioning \cite{ENISA2010}, some studies investigated how infrastructure sharing can help from an economic or operations perspective \cite{frisanco2008infrastructure, zheng2017economic}, increase rate coverage probability \cite{jurdi2018modeling, sanguanpuak2018infrastructure}, decrease energy consumption \cite{gambin2019sharing}, or distribute the load evenly over the network \cite{difranceso14}. 
{Next to improved resilience, infrastructure sharing plays a key role in the future of telecommunications to keep the services affordable in developing countries \cite{oughton2022policy, oughton2023policy} and to increase coverage \cite{arakpogun2020threading}.% although this only works if all participating MNOs invest fair and equally \cite{das2010determinants}. 
Therefore, nationwide infrastructure sharing might be difficult to achieve due to possible decrease in operator revenue~\cite{baake2021mobile}.
To mitigate this, one might consider to only share the infrastructure among certain operators, certain radio types~\cite{9121242} or on certain areas (Rural Access Network, \cite{oughton2022policy}). Please refer to \cite{ituTinfrasharing12} for an overview of different modes of infrastructure sharing, e.g., at the core network or radio access network.} {Note that virtualization techniques already implemented by Mobile Virtual Network Operators~\cite{liang2014wireless} can be considered for implementation of the specific national roaming scenario studied in this paper, i.e., a single MVNO having access to all resources of all national MNOs.}

% \textcolor{blue}{In our recent work, we compare national roaming as a back-up scenario to full national roaming in terms of coverage, capacity, and energy consumption~\cite{weedage2023national}.
% \lotte{Add something about virtual mobile network operators? Survey: \cite{blenk2015survey}}

Different from the studies that focus on infrastructure sharing \cite{panchal2013mobile, meddour2011role}, we focus on the special case of \textit{national roaming} where every user can use every existing BS of any MNO, { similar to the approaches in \cite{ENISA2010} and \cite{oughton2023policy}}. 
We investigate the entire network and focus on improving resilience instead of purely on maintaining higher capacity. 
Moreover, since our goal is to quantify the full potential of national roaming, rather than considering national roaming only as a backup implemented in exceptional cases such as post-disasters or for a single MNO, we explore it as a default mode of operation where all MNOs can use each other's network for serving the customers in the most efficient way.
Therefore, this can be considered as the best case scenario where all MNOs are in business agreement 
%
 { and operating with a shared core network}. 
 % {\color{red}Does it make sense to add this sentence? Do we really need a shared core network for our assumptions? Can we do the user association only in the RAN? I think we can, right? }
%
Note that the economic implications, e.g., settling the roaming costs, are beyond the scope of our paper. {Please refer to \cite{hou2020economics} for a thorough discussion on the economic aspects of infrastructure sharing.}


==> 3.system_model.tex <==
\section{System Model}\label{sec:system_model}

% NOTES: 
% Table 5 in \cite{hmamouche2021new} gives an overview of the key path loss models used in 5G. \cite{qingling2006rain} studies the attenuation in mmWaves due to rainfall (also in \cite{rappaport2013millimeter}). It might be useful to look at the system model of \cite{balakrishnan2019impact}, as this gives a complete model with beamforming, blockage and mobility.

 \begin{figure}
   \centering
    \includegraphics[width = 0.45\textwidth]{Figures/sysmodel.png}
    %{Figures/beam alignment-Page-2v2.png}
    \caption{An illustration of the considered system model with two MNOs, MNO$_{\textrm{1}}$ (with subscribers $u_1$ and $u_3$) and MNO$_{\textrm{2}}$ (with subscribers $u_2$ and $u_4$). MNO$_1$'s coverage hole can be filled with MNO$_2$'s base station BS$_3$ to serve $u_3$. Moreover, to have a stronger signal, $u_2$ can connect to MNO$_1$'s BS$_1$. } %https://drive.google.com/file/d/1MjbqGfxwQ6ghdQLvISsdpNe5UuRIpkPI/view?usp=sharing
    \label{fig:sysmodel}
\end{figure}
We consider a cellular network as in Fig.\ref{fig:sysmodel} consisting of a set of BSs denoted by $\B$ which operate at sub-6\,GHz bands. The network serves a set of users denoted by $\U$ and each user $u_i$ has a minimum rate requirement denoted by $C_i^{\textrm{min}}$ bits per second for its application to sustain a satisfying user experience.
%
If there is a link between user $u_i \in \U$ and BS$_j \in \B$, we denote this channel by $\ell_{ij}$. 
%Moreover, we will use superscript $b$ to denote BS related parameters while superscript $u$ will indicate the parameter being defined for a user. {\color{red} Do we use this?}

We consider two types of cell sites following the models in 3GPP~\cite{3gpp38901}: rural and urban macrocells. We model path loss according to the 3GPP TR 38.901 specification~\cite{3gpp38901} which defines path loss models for each listed cell type. For each case, line-of-sight~(LoS) and non-LoS path loss probabilities and models are defined in \cite[Table 7.4.1-1]{3gpp38901}. We denote the path loss at a receiver $u_i$ located at $r_{ij}$ meters away from the transmitter BS$_j$ by $\ploss(r_{ij})$. 
%{\color{red}Please refer to Fig.\ref{fig:3gpppathlo} for more details on the path loss models and the related parameters. }

We consider that a BS has a three-sector antenna and we adopt the 3GPP antenna gain model for these three-sector antennas~\cite{3gpp38901}. The horizontal antenna gain $A_H$ is defined as:
\begin{align}
    % A_V(\theta) &= -\min\left\{ 12 \left(\frac{\theta - 90}{\theta_{\text{3dB}}}\right)^2, 30\right\},\\
    A_H(\phi)[\text{dB}] &= - \min\left\{12 \left(\frac{\phi}{\phi_{\text{3dB}}}\right)^2, 20\right\},\label{eq:AH}
\end{align}
for horizontal misalignment angle $\phi$ (in degrees). 
%
The angle $\phi_{\text{3dB}}$ denotes the horizontal 3dB beamwidth. For three sector antennas, we assume $\phi_{\text{3dB}}=65\degree$\cite{rebato2019stochastic}. Thus, for user $u_i$ that connects to BS$_j$, the antenna gain is:
\begin{align}
    G_{ij}[\text{dB}] = G_{\text{max}} +A_H(\phi), \label{eq:antenna_gain_3GPP}
\end{align}
where $G_{\text{max}} = 20$ dB, which is the maximum attenuation. We assume users have omnidirectional antennas, and hence the receiver antenna gain is 0\,dB.


%\subsection{SINR and channel capacity} \label{subsec:sinr}
Now, let us denote the transmission power of BS$_j$ by $P_j$ and total noise over the transmission band by $N_{\text{tot}}$ which represents the sum of thermal noise power and noise figure of the receiver~\cite{halperin2013simplifying}. 
Then, the signal-to-interference-and-noise-ratio~(SINR) $\gamma_{ij}$ for $\ell_{ij}$ is defined as:
\begin{align}
    \gamma_{ij} = \frac{P_{j} G_{ij} \ploss(r_{ij})^{-1}}{N_{\text{tot}} +  I_{ij}}, \label{eq:snr}
\end{align}
where $G_{ij}$ denotes the antenna gain and $I_{ij}$ denotes the interference perceived by $u_i$ when it receives its downlink traffic from BS$_j$. %
Formally, $I_{ij}$ is defined as:
\begin{align}
    I_{ij} &= \sum_{m \in \B^j}P_{m} G_{im} \ploss(r_{im})^{-1}, \label{eq:interference}
\end{align}
where $\B^j$ is the set of BSs that operate on the same frequency as BS$_j$ and are within a radius of certain distance $r_\text{max}$ from BS$_j$.
%
We assume that the closest three BSs to BS$_j$ implement interference coordination schemes~\cite{hamzaicicsurvey13}. Hence, they do not interfere with BS$_j$.
% 
For a signal to be decodable with the lowest modulation scheme, we assume that the required minimum SINR is $\snir^{\textrm{min}}$. 

% {\color{red} Lotte: maybe we should say something about the fact that the interference calculation is in ratio and the rest is in dB?}


Finally, we can derive the channel capacity of user $u_i$ if it is connected to BS$_j$ (denoted by $C_{ij}$, Fig.~\ref{fig:sysmodel}).
%
We assume that the BS applies time-sharing among its served users. 
Then, the user's \textit{effective bandwidth}\footnote{We use the term \textit{effective bandwidth} to reflect the bandwidth the user will experience if it is served a certain amount of time in the available bandwidth, i.e., $\effectiveRes_{ij}$. 
Hence, the effective bandwidth is $\effectiveRes_{ij} W_j$.} will be only a fraction $\effectiveRes_{ij}$ of the total bandwidth $W_j$. 
Consequently, we can calculate the maximum achievable throughput $C_{ij}$ as:
\begin{align}
   C_{ij} = \effectiveRes_{ij}W_j\log_2(1 + \gamma_{ij}).\label{eq:channel_capacity}
\end{align}
%We calculate $\effectiveRes_{ij}$ by assuming that every user is allocated a fraction of resources proportional to its rate requirement.
%using proportionally-fair resource allocation algorithm~\cite{banchs2007proportional}, 
%where we calculate $\effectiveRes_{ij}$ based on the minimum rate requirement of a user~($C^\text{min}_i$) and the spectral efficiency of a user SE$_{ij}= \log_2(1 + \gamma_{ij})$. Then, each BS determines $\effectiveRes_{ij}$ as follows:
%\begin{align}
%    % \effectiveRes_{ij}= \left(\text{SE}_i \cdot \sum_{k\in \mathcal{U}^j} \frac{1}{\text{SE}_k}\right),
%    \effectiveRes_{ij} &= \theta_j %\frac{C^\text{min}_i}{\text{SE}_i},\label{eq:effective_bandwidth}.
%\end{align}
Now, let us discuss how to determine  $\effectiveRes_{ij}$. 
Ideally, each user should be served for a minimum amount of time such that its rate requirement $C^\text{min}_i$ is met. Let us denote this minimum  effective bandwidth by $W^{\textrm{min}}_{ij}$ that is needed to ensure 
$C^\text{min}_i$. We can calculate $W^{\textrm{min}}_{ij}$  as follows:
\begin{align}
W^{\textrm{min}}_{ij} = \frac{C^\text{min}_i}{\log_2(1 + \gamma_{ij})}.
\end{align}
Since the total requested effective bandwidth by all users might exceed the available bandwidth $W_j$, for the sake of fairness among all users, each user is assigned effective bandwidth proportionally to its need $W^{\textrm{min}}_{ij}$. Hence, we set $\effectiveRes_{ij}$ as follows:
\begin{align}
    \effectiveRes_{ij} = \frac{W^{\textrm{min}}_{ij}}{\sum_{k\in\U^j} W^{\textrm{min}}_{kj}},\label{eq:effective_bandwidth}
\end{align}
% where $\theta_j$ is a normalizing constant to ensure that the sum of $\effectiveRes_{ij}$ values is 1 to reflect the total resources~(e.g., time) available for use. 
 %the total bandwidth of BS$_j$ sums to $W_j$.
%For a channel with bandwidth $W_j$, $\theta_j$ is calculated as follows: \begin{align}
%   \theta_j &=  {\frac{\sum_{k\in\U^j}\frac{C^\text{min}_k}{{\text{SE}_k}}}{W_j}}, 
%\end{align}
%{\color{brown}($\text{SE}_i$ is in bps/Hz, right?! then, I think that here either we consider $C^\text{min}_k$ also in bps/Hz or we add $W_j$ in $\text{SE}_i$. Did I understand it correctly? Here $\theta_j$ implies that if there is no enough bandwidth for meeting all users requirements, then allocate all the available bandwidth proportionally to the requested data rates and $\frac{C^\text{min}_i}{\text{SE}_i}$ means the fraction of the total bandwidth to satisfy user $i$, which should not have any unit. However, case $C^\text{min}_i$ is in [bps], then $\frac{C^\text{min}_i}{\text{SE}_i}$ is in [Hz], right?!)}
where $\mathcal{U}^j$ denotes the set of users connected to BS$_j$. When $\sum_{i\in\U^j} W^{\textrm{min}}_{ij} \leqslant W_j$, the bandwidth is sufficient for all connected users and users  maintain at least their requested rate. %
Otherwise, users are assigned effective bandwidth proportional to their $W^{\textrm{min}}_{ij}$ with respect to the needed bandwidth by all users, i.e.,  $\sum_{i\in\U^j} W^{\textrm{min}}_{ij}$. \newInfo{Note that we consider data services in this paper, hence our metric to represent user satisfaction is based on the user's data rate. However, for other services requiring guaranteed latency or reliability, one would need different metrics for measuring performance and consequently resilience.}

We assume that active users are distributed by a Poisson Point Process with given density according to the population density. As the user association scheme, we assume that a user connects to the BS that offers a high SINR that is above a threshold SINR~($\gamma^{\text{min}}$) with the lowest number of users connected to it. We iteratively connect a randomly-chosen user $u_i\in \U$ to $\text{BS}_{\text{opt}}$ where  $\text{BS}_{\text{opt}}$ is: 
\begin{align}
    \text{BS}_{\text{opt}} = \argmax_{j\in \B}\frac{
    %\text{SINR}
    \gamma_{ij}}{D_{\text{BS}_j}},  
    \label{eq:user_association}
\end{align}
where %SINR$_{ij}$ denotes the link-SINR for channel $\ell_{ij}$ and 
$D_{BS_j}$ is the number of users connected to BS$_j$. 
Finally, we denote by $X=[x_{ij}]$ the association state of $u_i$ with BS$_j$ where $x_{ij}$ yields value 1 if $u_i$ is associated with BS$_j$ and zero otherwise. 
%Finally, we will denote by $\rate_{ij}$ the achieved theoretical capacity of the channel $\ell_{ij}$ and the minimum rate requirement of $u_i$ by $\rate^{\textrm{min}}_i$.

==> 4.resilience_analysis.tex <==
\section{Two metrics to assess network resilience}\label{sec:res_metrics}
%
% \textcolor{blue}{General comment: We should think on where and how we use resilience. I think that for example the metrics we introduce are not really resilience metrics by themselves (but performance measures), they only become resilience metrics when we investigate them under failures. }

As described in Sec.~\ref{sec:related}, resilience can be measured both using topological metrics and functional metrics. However, none of the discussed metrics in Sec.~\ref{sec:related} reflect what resilience implies for the citizens, i.e., customers of an MNO. %
For a cellular network, two properties are key to assess performance: coverage and capacity. For the coverage, we quantify the \textit{fraction of disconnected population} (per province/city) as a performance metric. We will refer to this metric as FDP. We assume that a user is disconnected from the network if its received signal strength is too low to decode the signal with the most robust modulation~(e.g., BPSK). 
%
Note that this metric is an adapted version of SINR coverage that is typically used for capacity analysis in cellular networks, e.g., \cite{rebato2019stochastic}.

To measure capacity, we will use the throughput that a user maintains. However, since functional metrics describe the level of service that users experience, it depends on their application requirements. 
%
Indeed, cellular networks can support many applications with vastly different rate requirements, which also impacts the satisfaction level of a user with a given throughput. Therefore, we  quantify the \textit{fraction of satisfied population} (per province/city) and refer to it as FSP. 
%
A user is \textit{satisfied} if the user is connected to the network~(i.e., it is not in the disconnected population) and the provided throughput to this user is above the minimum rate requirement of the used application. 
%
Note that applications can be diverse, e.g., URLLC or mMTC services in 5G networks require a low data rate but can assert strict latency or reliability performance \cite{8476595}. 
In this study, we consider only the rate requirements in defining our satisfaction metric. 

%Let us denote by $X=[x_{ij}]$ the association state of $u_i$ with BS$_j$ where $x_{ij}$ yields value 1 if $u_i$ is associated with BS$_j$ and zero otherwise. For a signal to be decodable with the lowest modulation scheme, the required SINR is denoted by $\snir^{\textrm{min}}$. Finally, we will denote by $\rate_{ij}$ the achieved theoretical capacity of the channel $\ell_{ij}$ and the minimum rate requirement of $u_i$ by $\rate^{\textrm{min}}_i$. \lotte{Maybe this paragraph should go to system model?}
% 

Now, we can define FDP and FSP formally. Let us denote whether $u_i$ is disconnected from the network by $\delta^{\fdp}_{i}$. We define it as follows:  
\begin{align}
\delta^{\text{fdp}}_{i} = \begin{cases}
    1 & \textrm{if}  \sum\limits_{j\in \B}\snir_{ij}x_{ij} \leqslant \snir^{\textrm{min}} \\
    0 & \textrm{otherwise}.
\end{cases}
\end{align}
Then, we can calculate the network's coverage performance in terms of fraction of disconnected population as: 
\begin{align}
\FDP = \frac{\sum_{i\in|\U|} \delta^{\fdp}_i}{|\U|}.
\end{align}

For FSP, we denote the satisfaction status of $u_i$ by $\delta_i^{\fsp}$ and define it as follows:
\begin{align}
\delta^{\fsp}_{i} = \begin{cases}
    1 & \textrm{if} \sum\limits_{j\in |\B|}\rate^s_{ij}x_{ij} \geqslant \rate^{\textrm{min}}_i { \textrm{ and } } {\color{black}\delta^{\text{fdp}}_{i} = 0}\label{eq:fsp_1} \\
    0 & \textrm{otherwise}.
\end{cases}
\end{align}
Similarly, the FSP can be defined as: $\FSP = \sum_{i\in|\U|} \delta^{\fsp}_i / |\U|$. As stated in (\ref{eq:fsp_1}), a precondition for satisfaction is being connected. In other words, $u_i$ must have a signal from BS$_j$ with a strength that is higher than $\snir^{\textrm{min}}$ and the perceived throughput must be at least $\rate^{\textrm{min}}_i$ bps. 

% Additionally, to assess the importance of a BS for the network, we introduce $\Delta_j^\fsp$ that quantifies the decrease in FSP due to the failure of BS$_j$. More formally, we define $\Delta_j^\fsp$ as:
% \begin{align}
%     \Delta_j^\fsp = \frac{\sum_{i \in |\U|}{\delta_i^\fsp - \tilde{\delta}_i^\fsp}(j)}{|\U|},\label{eq:delta_failure}
% \end{align}
% where $\tilde{\delta}_i^\fsp(j)$ is the FSP after failure of BS$_j$. We define $\Delta_j^\fdp$ in a similar fashion.

%\textcolor{red}{SB: can we formally define a metric which shows importance of a BS for resilience? a metric quantifying in a way how would the resilience metrics be affected if this BS fails?}
\smallskip






==> 5.performance_evaluation.tex <==
\section{Dutch cellular networks as a case study}\label{sec:perfeval}
In this section, we first introduce the datasets and model parameters we use to simulate the considered cellular networks. 
Afterwards, we provide an analysis of the current state of the network in terms of FDP and FSP performance, and show characteristics of the three main operators in the Netherlands.
%
% Finally, we present in Section \ref{subsec:perf-strategies} a performance analysis of our proposals to improve the resilience of a cellular network in these identified regions.

\subsection{Datasets and simulation setting}
\label{sec:data}

\textbf{Antenna dataset:} We use the Dutch Telecommunication Authority's~({\color{black}Rijksinspectie Digitale Infrastructuur}) antenna registration dataset~\cite{antenneregister}, which includes the following information for each BS registered in the dataset: technology~(2G, 3G, 4G, 5G), location, center frequency, effective radiated power~(ERP) per channel, antenna height and antenna sectors. 
As Fig.~\ref{fig:BS_example} shows, BSs typically operate using three sector antennas, whose antenna gain model is introduced in Sec.~\ref{sec:system_model}.
%
%\textbf{Sectorized antennas:}
%Most of the BSs in the dataset have three-sector antennas. 
To calculate the gain of these antennas, we use the antenna radiation pattern as given in the 3GPP TR 36.942 specification~\cite{access2020radio}. The main direction in which the antennas transmit is available in the data set. 
%
Since the dataset includes the effective isotropic radiated power (EIRP), we assume that this power already includes $G_{\text{max}}$ in \eqref{eq:AH}. 
%
Thus, to obtain $G_{ij}$, we only add \eqref{eq:AH} from the given EIRP.
%
The horizontal boresight angle of all antennas is given in the dataset.
%
We remove the omnidirectional antennas in the dataset, as manual investigation showed that these antennas are mostly placed indoors, and some MNOs choose to not register these antennas in the dataset \cite{antennekaart}. These removed data correspond to $5.3\%$ of the 3G, 4G and 5G BSs.
%
Moreover, we have removed BSs with 2G technology~(corresponding to $29\%$ of all BSs) from the dataset as 2G network serves a different purpose, e.g., such as smart metering, rather than voice or data communications. Moreover, 2G networks will be phased-out in the near future in the Netherlands~\cite{2gphasedout}.  

\begin{figure}
    \centering
    \includegraphics[width = 0.42\textwidth]{Figures/Resilience_Damstraat.pdf}
    %{Figures/Amsterdam_small.png}
  %  \caption{An example entry from the data set. For every BS, the following information is available: the \textit{provider}, \textit{plaats}~(location), \textit{hoogte} (height), \textit{hoek}~(angle), \textit{frequentie}~(frequency) and \textit{vermogen}~(power)~(netwerkleverancier), reproduced from~\cite{antennekaart}. }
     \caption{An example entry from the data set. For every BS, the following information is available: the  provider, place, height, angle, frequency,  power, \newInfo{reproduced from}~\cite{antennekaart}. }
    \label{fig:BS_example}
\end{figure}


\textbf{Mobile network operators:}
\newInfo{The Netherlands has three MNOs: KPN, Vodafone, and Odido~(previously, T-Mobile). Additionally, many virtual MNOs use the infrastructure of these three operators. 
As the antenna data set does not provide data on the owner of each BS, we map each BS to one of the three MNOs based on the frequency range that each MNO owns \cite{frequentieoverzicht} (Table \ref{tab:frequency_statistics}). Our dataset includes information on the three MNOs which we refer to in this study as \KPN, \TMobile, and \Vodafone, in no particular order. Table \ref{tab:frequency_statistics} also shows the number of BSs of these three MNOs.  }
%  \lotte{Maybe remove last column of Table~\ref{tab:frequency_statistics}? Or give explanation about realistic divisions?}
%  proportional to the percentage of the number of BS every MNO has. This information can be found in the last column of Table~\ref{tab:frequency_statistics}.  
%
As can be seen from the operation frequencies listed in Table~\ref{tab:frequency_statistics}, at the time of this study, 5G deployments operate only in the low-band ($<$ 1 GHz) and mid-band 5G spectrum, i.e., 1 GHz to 2.6 GHz. Higher frequencies, such as 3.5 GHz, are expected to become available after an auction in December 2023\footnote{\url{https://www.rijksoverheid.nl/actueel/nieuws/2022/05/12/adviescommissie-35-ghz-band-in-2023-in-gebruik-voor-mobiele-communicatie}}. 
We believe that our analysis can also provide insights to the MNOs on where the higher frequency cells should be deployed for capacity and coverage improvement. 
%
% Fig.~\ref{fig:BS_example_enschede} illustrates the BS deployment of the municipality of Enschede for each provider.

\begin{table*}[]
\centering
\caption{Frequency bands and number of BSs per provider for 3G, 4G and 5G technologies.}
\label{tab:frequency_statistics}
\renewcommand{\arraystretch}{1.2}
\resizebox{1.8\columnwidth}{!}{%
\begin{tabular}{|l|lllc|llll|}
\hline
 &
  \multicolumn{4}{c|}{Centre frequency and bandwidth in MHz} &  \multicolumn{4}{c|}{Number of BSs}\\
 &
  \multicolumn{1}{c}{3G} &
  \multicolumn{1}{c}{4G} &
  \multicolumn{1}{c}{5G} & 
  \multicolumn{1}{c|}{Total (MHz)} & 
  \multicolumn{1}{c}{3G} &
  \multicolumn{1}{c}{4G} &
  \multicolumn{1}{c}{5G} &
  \multicolumn{1}{c|}{Total}   \\ \hline
\KPN &
942.2 (5), 2152.6 (5) &
  \begin{tabular}[c]{@{}l@{}}816 (10), 1474.5 (15), 1815 (20), \\ 2160 (20), 2605 (30), 2660 (10)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}773 (10), \\ 2160 (20)
  \end{tabular}  & 175 &4716 &4621 &3508 &12845 \\ \hline 
\TMobile &
 957.4 (5),  2137.4 (10) &
  \begin{tabular}[c]{@{}l@{}}796 (10), 950 (10), 1487 (10), \\ 1850 (10), 1860 (30), 1865 (20), \\ 2137.5 (15), 2580 (20), 2652 (4),\\ 2572.5 (15), 2672.5 (15), 2675 (20)\end{tabular} &
  783 (10) & 204   & 4752      & 4855   & 3590    & 13197   \\ \hline 
\Vodafone & \quad\quad\quad\quad---
  &
  \begin{tabular}[c]{@{}l@{}}763 (10), 806 (10), 1459.5 (15), \\ 1835 (20), 2117.5 (15), 2120 (20), \\ 2630 (20), 2644.4 (10)\end{tabular} &
  1835 (20)& 140  & 0   & 4477   & 3395   & 8313 \\ \hline
\end{tabular}%
}
\end{table*}

\textbf{BS transmission power:} The power provided in the dataset is the maximal EIRP that the BS can transmit~(in dBW), which is an upper bound on the EIRP that will actually be used. 
Comparing the values with the reported values in \cite{deruyck2014power} which are collected from data sheets of 
network equipment manufacturers, we infer that the power values in the dataset represent the total power budget of a BS which is used for also other tasks such as air cooling or digital signal processing. Hence, we assume that every BS operates using $90\%$ of its maximum power recorded in the dataset. {We have observed no significant differences in the power levels of different MNOs.}

\textbf{Rate requirements:}
In a cellular network, users can have different rate requirements based on their application. %Since the 5G network is not yet functional in the Netherlands.
% 
To represent the rate requirements, we assume a varying rate requirement, where each user gets assigned a rate requirement $C^\text{min}$ that is uniformly distributed in [$R_{\text{min}}$, $R_{\text{max}}$] Mbps.


\textbf{Population density for each $\mathbf{500\times500}$m square:}
To simulate the population, we use the data from Statistics Netherlands~(Centraal Bureau voor Statistiek)\cite{cbs}, which records the number of inhabitants per $500\times500$m square in the Netherlands and the \textit{urbanity} of this area {\color{black} at the end of 2020}. 

The urbanity data distinguishes between five levels of urbanity, where level-1 represents the highest address density and level-5 the lowest. More precisely, the \textit{area address density} quantifies the number of addresses within a circle with a radius of one kilometer around an address divided by the area of the circle\footnote{\url{https://www.cbs.nl/nl-nl/onze-diensten/methoden/begrippen/stedelijkheid--van-een-gebied--}.},
%
and distinguishes the following intervals for the urbanity levels: 
\begin{itemize}
  \item level-$1$ above 2500 per km$^2$;
  \item level-$2$ in [1500, 2500) km$^2$; 
  \item level-$3$ in [1000, 1500) per km$^2$; 
   \item level-$4$ in [500, 1000) km$^2$; 
\item level-$5$ lower than 500 per km$^2$.
\end{itemize}

Based on the urbanity level of the area in which a BS is located, we determine whether it is an urban macrocell~(UMa) or a rural macrocell~(RMa). 
%We classify two different cells as described in Figure \ref{fig:sysmodel}{\color{red} change figure?} based on the address density of a zip code.  
We assume that an urbanity level of $1\,-3$ corresponds to the UMa scenario and levels 4 and 5 are rural areas (RMa). 

We assume that a fixed fraction $f_p$ of the population is active at a time and therefore $1-f_p$ fraction of the population uses other connectivity modes such as Wi-Fi or is not connected to a mobile network.  We simulate users in these $500 \times 500$m squares by a homogeneous Poisson point process with a fraction $f_p$ of the population density as intensity measure. As the number of customers for each MNO is not publicly available, we equally divide the users among the MNOs.\footnote{Based on Tables~\ref{tab:frequency_statistics} and \ref{tab:municipality_province_statistics}, one might conclude that an equal distribution among MNOs would not be fair. We also have studied a different user distribution: $40\%/40\%/20\%$ for MNOs 1, 2 and 3 and for this distribution the trend in the results stayed the same.}

 
% \begin{figure*}[thb]
%     \centering
%     \subcaptionbox{\KPN\label{sfig:KPN}}{\includegraphics[width=.30\textwidth]{Figures/EnschedeKPN_BSs.png}}\hfill
%      \subcaptionbox{\TMobile\label{sfig:TMobile}} {\includegraphics[width=.30\textwidth]{Figures/EnschedeT-Mobile_BSs.png}}\hfill
%     \subcaptionbox{\Vodafone.\label{sfig:Vodafone}}{\includegraphics[width=.30\textwidth]{Figures/EnschedeVodafone_BSs.png}}\hfill
%     \caption{BS deployment in Enschede for the three MNOs.}\label{fig:BS_example_enschede}
% \end{figure*}

\begin{table}[t]
\centering
\renewcommand\arraystretch{1.2}
\caption{Default parameters used in simulations.}
\label{tab:sim-params}
\begin{tabular}{|l|l|} \hline 
Parameter& Value(s)\\ \hline
Rate requirement $R_{\text{min}} - R_{\text{max}}$& 8 - 20 Mbps \\ \hline
Minimum SINR $\snir^\text{min}$ & 5 dB \\ \hline
Fraction of active population $f_p$ & $2\%$\\ \hline
Maximum distance for interference $r_\text{max}$ & $5$ km\\ \hline
\end{tabular}
\end{table}

\begin{figure*}[thb]
    \centering
   \subcaptionbox{Number of BSs per km$^2$.\label{sfig:bs_per_area_provinces}}{\includegraphics[width=.45\textwidth]{Figures/BSperArea_provinces.pdf}\hfill}\label{fig:statistics_regions}
    \subcaptionbox{Number of active users per BS.\label{sfig:user_per_BS_provinces}}{\includegraphics[width=.45\textwidth]{Figures/usersPerBS_provinces.pdf}}
    \caption{Number of users per BS and BS density (km$^2$) per province.} 
    %\textcolor{blue}{This is to give us some guidelines when comparing cities, MNOs. It is apparent that MNO-3 has the highest number of users and the least number of BSs. not reflected here, but the lowest frequency bands too. Hence, not surprising that its performance is the poorest.} \lotte{But even with a more fair division of users over MNOs, MNO-3 did perform the poorest..}  
\end{figure*}

\textbf{Failures:} To measure the resilience of the network, we simulate two types of failures: \textit{isolated} and \textit{correlated} failures. 
Technology-related failures or cyber attacks on the network can be modeled as \textit{isolated} failures, where every BS fails independently and with probability $p_{iso}$. 
Disasters such as earthquakes and hurricanes often only impact a specific geographic area. Therefore, they affect the performance of several nearby network links.
For this reason, we model this as \textit{correlated failures} where link within and close by the disaster area fail. 
We pick the center of the simulated area as center of impact, and let all BSs that are within radius $r$ meter of this center fail~\cite{agarwal2013resilience}.
% Next to that, we analyse how the network is affected by a higher user load impacts by increasing the percentage of active users $f_p$. 
%In this setting, we change the intensity of the Poisson Point Process that we use to simulate users. 

 
\subsection{Current state of the networks} \label{subsec:perf-current}
Using the described datasets, we first investigate each MNO's performance separately without any failures using the FSP and FDP metrics. Next to that, we show some statistics about the current deployments, e.g., the number of users per BS or the number of BSs per km$^2$. 
%
We also consider a scenario with national roaming in which all networks work together to serve the users and each user can connect to the BS which provides the best performance according to (\ref{eq:user_association}). 
%Our analysis aims at addressing the following questions:
%\begin{itemize}
%\item What is the FDP and FSP performance of Dutch cellular networks in different regions of the Netherlands? 
%\item What would be the achieved FSP and FDP if all cellular operators act as a single national MNO, i.e., if national roaming were possible? In which cities/regions will this provide the highest gains? 
%\end{itemize}

Table~\ref{tab:sim-params} provides the default values of the parameters used in the simulations. In our evaluation, \newInfo{ we set $f_p=2\%$ to keep the average number of users per BS around $10$ \cite{george2018distribution}.}
Moreover, 
we consider $R_{\text{min}}=8$\,Mbps as the Dutch regulatory body asserts that each MNO must provide at least 8 Mbps outdoor data rate in each region~\cite{min8mbps}. \newInfo{As $R_{\text{max}}$, we choose $20$ Mbps considering the recommended application rate requirement in the literature, e.g., average 20 Mbps for mobile gaming\footnote{NordVPN \url{https://nordvpn.com/blog/internet-speed-for-gaming/}}.} 
%
Then, when users are associated to a BS, the BS calculates the effective bandwidth $\effectiveRes_{ij}$ per user according to \eqref{eq:effective_bandwidth}. 

\begin{table}[t]%bh]
\renewcommand{\arraystretch}{1.05}
\caption{Statistics 
%per municipality for the selected 10 municipalities~(from AL to MI) and 
of the 12 Dutch provinces.% of the Netherlands~(from DR to ZH).
\label{tab:municipality_province_statistics}}
\begin{tabular}{|l|ccc|c|c|c|}\hline 
   & \multicolumn{3}{c|}{Number of BSs}                                       & \multirow{2}{*}{\#users} & \multirow{2}{*}{Avg.urb.} & \multirow{2}{*}{Area, km$^2$}\\
   & \KPN & \TMobile & \Vodafone &                          &                           &      \\ \hline
% AL & 182                 & 196                     & 130                      & 1567                     & 2.9                       & 163.7                          \\
% AM & 750                 & 888                     & 485                      & 5885                     & 1.7                       & 195.0                          \\
% DH & 517                 & 632                     & 289                      & 3266                     & 1.2                       & 85.2                           \\
% EI & 332                 & 429                     & 206                      & 1651                     & 2.0                       & 84.7                           \\
% EL & 73                  & 61                      & 32                       & 223                      & 4.5                       & 56.8                           \\
% EM & 111                 & 112                     & 65                       & 1126                     & 4.4                       & 347.3                          \\
% EN & 220                 & 254                     & 131                      & 1320                     & 2.6                       & 142.6                          \\
% GR & 479                 & 509                     & 377                      & 6083                     & 2.9                       & 197.8                          \\
% MA & 166                 & 147                     & 115                      & 893                      & 2.1                       & 60.4                           \\
% MI & 71                  & 83                      & 61                       & 383                      & 2.9                       & 50.9   \\              \hline 
DR & 337  & 345 & 223 & 6558  & 4.7 & 2691  \\ 
FL & 212  & 218 & 131 & 4089  & 3.5 & 1471  \\ 
FR & 272  & 346 & 214 & 6586  & 4.6 & 3555  \\ 
GE & 1508  & 1334 & 856 & 22877  & 4.0 & 5145  \\ 
GR & 291  & 330 & 247 & 1761  & 4.4 & 2378  \\ 
LI & 986  & 863 & 590 & 10859  & 4.0 & 2214  \\ 
NB & 1773  & 1818 & 1081 & 24947  & 3.7 & 5076  \\ 
NH & 1538  & 1723 & 1008 & 23215  & 3.1 & 2875  \\ 
OV & 760  & 783 & 471 & 14292  & 4.0 & 3427  \\ 
UT & 841  & 820 & 498 & 11646  & 3.1 & 1562  \\ 
ZE & 244  & 294 & 187 & 4716  & 4.5 & 1889  \\ 
ZH & 1931  & 2311 & 1244 & 28991  & 2.5 & 2865  \\ \hline
\end{tabular}
\end{table}
% First, we investigate the SNR and capacity distributions for different regions in the Netherlands without any rate requirement or minimum SNR. 
%

{Each simulation is repeated 100 times for statistical significance as user locations and path loss are random.} We provide simulations of the performance of national roaming on the province level.  Table~\ref{tab:municipality_province_statistics} provides an overview of different properties of all provinces. 
Fig.~\ref{sfig:bs_per_area_provinces} shows the BS density per km$^2$ in each province. We can observe clear differences across provinces and among MNOs. 
First, \Vodafone~has the lowest BS density due to its significantly lower number of BSs as highlighted in Table~\ref{tab:municipality_province_statistics}. As expected, ZH as the most populated province~(including Amsterdam) has the highest BS density. Comparing \KPN and \TMobile, we do not observe a significant difference.  Fig.~\ref{sfig:user_per_BS_provinces} shows the higher user density per BS for \Vodafone in all provinces compared to \KPN and \TMobile due to its less dense BS deployment. 


\section{Performance analysis} %\color{blue} National roaming

With these insights on the infrastructure of each MNO, now, let us discuss the coverage and capacity performance of these MNOs. Fig.~\ref{fig:FDPFSP} shows the FSP and FDP per province per MNO and for all MNOs together, representing the case where all operators can use each other's network as in national roaming. 
%
Looking closer at Fig.~\ref{sfig:FDP}, we have the following three observations. \textit{First}, in various regions, some operators fail to provide sufficient SINR to their customers, resulting in an FDP as high as 0.11 in Friesland or around 0.09 %0.086
in Zeeland. 
%
Especially in these regions, national roaming provides its benefits as reflected in a significant improvement in FDP with an achieved FDP of zero. Moreover, \TMobile consistently achieves a higher performance in almost all regions compared to \KPN, whose performance is in turn significantly better than \Vodafone. 
We attribute this superior performance of \TMobile to its higher spectrum resources~(204 MHz vs. 175\,MHz and 140\,MHz) as we have not observed a significant difference in their BS density in Fig.~\ref{sfig:bs_per_area_provinces}. The performance gap between \Vodafone and other MNOs can emerge due to the lower spectrum resources and lower BS density. 
%


When it comes to FSP, Fig.~\ref{sfig:FSP} again shows a superior performance of \TMobile. However, the achieved FSP varies between $0.73$ and $0.89$, indicating a need for performance improvement. Comparing \KPN and \Vodafone, generally speaking, \KPN outperforms \Vodafone in terms of FSP, except in Friesland, which is one of the worst-performing regions in terms of both FSP and FDP. 
These low-FSP regions could be considered as initial places for investment to ensure higher user satisfaction. Also, \KPN and \Vodafone provide a more varying FSP across provinces compared to \TMobile. For example, the achieved FSP for \TMobile ranges from $0.70 - 0.95$, while for \KPN and \Vodafone, the achieved FSP lies in $[0.54, 0.89]$ and $[0.56,0.80]$, respectively. This large range in satisfaction might emerge as a result of different deployment strategies.
%



\begin{figure*}[thb]
    \centering
    \subcaptionbox{FDP\label{sfig:FDP}}{\includegraphics[width=.33\textwidth]{Figures/FDPprovinces.pdf}}\hfill
     \subcaptionbox{FSP\label{sfig:FSP}} {\includegraphics[width=.33\textwidth]{Figures/FSPprovinces.pdf}}\hfill
    \subcaptionbox{Gains of each MNO from national roaming.\label{sfig:FDP_gains}}{\includegraphics[width=.33\textwidth]{Figures/province_difference.pdf}}\hfill
    \caption{FDP, FSP, and achieved gains from national roaming for the three MNOs in different provinces.} % Scenario-\textit{All} corresponds to the case where all network infrastructure is used to serve the users, i.e., national roaming.} 
    \label{fig:FDPFSP}
\end{figure*}

% \begin{figure*}[thb]
%     \centering
%     \subcaptionbox{FDP\label{sfig:FDP_cities}}{\includegraphics[width=.33\textwidth]{Figures/FDPmunicipalities.pdf}}\hfill
%     \subcaptionbox{FSP \label{sfig:FSP_cities}}{\includegraphics[width=.33\textwidth]{Figures/FSPmunicipalities.pdf}}\hfill
%     \subcaptionbox{Gains of each MNO from national roaming.\label{sfig:city_gains}}{\includegraphics[width=.33\textwidth]{Figures/municipality_difference.pdf}}\hfill
%     \caption{FDP, FSP, and achieved national roaming gains in select 10 municipalities. Fig (c) shows the improvement in FSP and FDP with national roaming of all municipalities of the Netherlands, not only the 10 municipalities shown in (a) and (b).} 
%     \label{fig:FDPFSP_municipalities}
% \end{figure*}
\textit{Second}, letting users connect to every BS regardless of their MNO improves FSP consistently as expected. This improvement is, however, more significant in some regions such as Friesland or Overijssel. % 
%
\textit{Third}, national roaming improves FSP by around $0.05-0.35$ in absolute terms~(Fig.~\ref{sfig:FDP_gains}). However, in contrast to FDP, it does not yet suffice to meet all rate requirements as reflected by FSP always being below $1.0$. This can be considered as an indication of the need for infrastructure expansion or for more advanced schemes to provide higher throughput, e.g., expanding to higher spectrum bands with abundant bandwidth. 
%
When it comes to gains experienced by each MNO in the case of national roaming, Fig.~\ref{sfig:FDP_gains} plots the performance gain in terms of FDP and FSP observed by each MNO. In line with our earlier observations, \Vodafone benefits the most from national roaming, followed by \KPN with a slight difference over \TMobile. Please note that despite $\Delta$FDP being very narrow for \KPN and \TMobile, the resulting FSP gain is still remarkable also for these operators.
%
Note that all $\Delta$FSP and $\Delta$FDP values in Fig.~\ref{fig:FDPFSP} are positive implying that national roaming does not lead to performance degradation  and even the best-performing MNO can benefit from it, albeit less significantly compared to other MNOs with less-dense deployment. 
%
{As a nation-wide implementation of national roaming requiring collaboration of all MNOs and technologies might be hard to realize, we also investigated roaming in a limited way to provide insights to the MNOs and  when and where they could benefit most from national roaming. Such an analysis could also help national telecommunication regulatory bodies to develop policies enforcing national roaming for serving the underserved areas or regions benefiting the most from this mode of operation. We focused on the following questions}\footnote{In a recent work, we also compared national roaming as considered in this paper with current implementation of national roaming where MNOs only can use others' network when they experience a failure in their own network, i.e., as a fallback strategy. Please refer to \cite{weedage2023national} for more details.}: {(i) which cellular technology, i.e., 3G, 4G or 5G, should be prioritized for roaming if MNOs are eager to develop such roaming agreements? and (ii) in which areas should the MNOs consider roaming agreements, i.e., rural areas where the infrastructure is less dense or in urban areas where the population density thereby the traffic load is higher?  }


% and (iii) which MNOs should implement bilateral roaming agreements similar to current regulations allowing roaming as a fall-back strategy in the event of service loss?} 

%To do so, we analyzed the performance of national roaming of specific technologies, such as only sharing one technology (3G, 4G or 5G, Fig.~\ref{fig:technology_Enschede}), 
%implement national roaming only in one area (UMa and RMa, as defined in \cite{3gpp38901}, Fig.~\ref{fig:area_Enschede}) or using national roaming as a fall-back \cite{weedage2023national}.} 


% Fig.~\ref{fig:technology_Enschede}) 

\begin{figure*}[thb]
    \centering
    \subcaptionbox{FDP\label{sfig:technology_fsp}}{\includegraphics[width=.45\textwidth]{Figures/FDP_technologies_Amsterdam.pdf}}\hfill
    \subcaptionbox{FSP \label{sfig:technology_fdp}}{\includegraphics[width=.45\textwidth]{Figures/FSP_technologies_Amsterdam.pdf}}\hfill
    \caption{FDP and FSP in Amsterdam under only roaming for a specific technology~(5G, 4G or 3G).  
    } 
    \label{fig:technology_Enschede}
\end{figure*}



{Fig.~\ref{fig:technology_Enschede} depicts the resulting FDP and FSP when operators only share BSs of a certain technology to serve each other's users. In this case, users access to the network of their own operator for the remaining technologies for which national roaming is not implemented. Moreover, we compare this to the scenario with sharing all technologies (`3G, 4G and 5G'). This figure shows that only sharing the 4G LTE technology performs similar to the full national roaming approach, and even slightly better in terms of FSP for \KPN and \Vodafone. Only sharing 5G NR or 3G UMTS performs significantly worse, both in terms of FDP and FSP. We speculate that the superiority of 4G LTE can be explained by the large spectrum resources (Table \ref{tab:frequency_statistics}), as this will result in the least interference. For \KPN, while 36\% of the cell sites are 4G LTE sites, the spectrum for these areas accounts for 60\% of the spectrum used by this operator. For \TMobile, 40\% of the cell sites are 4G operating on 88\% of the spectrum owned by \TMobile. Lastly, for \Vodafone, 4G cell sites correspond to 54\% of the cell sites and the spectrum allocated to these cells is 86\%. }

\begin{figure*}[thb]
    \centering
    \subcaptionbox{FDP\label{sfig:area_fsp}}{\includegraphics[width=.45\textwidth]{Figures/FDP_areas_Amsterdam.pdf}}\hfill
    \subcaptionbox{FSP \label{sfig:area_fdp}}{\includegraphics[width=.45\textwidth]{Figures/FSP_areas_Amsterdam.pdf}}\hfill
    \caption{FDP and FSP in Amsterdam for only sharing in specific cell types (UMa or RMa).} 
    \label{fig:area_Enschede}
\end{figure*}

{For addressing (ii), we considered roaming only in UMa or RMa cells as defined in \cite{3gpp38901} as these two cells correspond to urban areas and rural areas, respectively. Fig.~\ref{fig:area_Enschede} illustrates FDP and FSP when sharing is applied only in certain areas. This figure shows that sharing infrastructure in the UMa areas outperforms sharing in RMa areas significantly. We attribute this result to the number of resources: for all operators, there are 5-6 times more BSs classified as UMa compared to RMa. Moreover, the population is concentrated in urban areas resulting in higher traffic load. 
A clear recommendation on whether MNOs should prioritize sharing a certain technology or sharing in certain areas is not straightforward as our results suggest that sharing more resources (either spectrum or BS locations) are expected to result in better FDP and FSP. }

\textbf{User association: }
{Fig.~\ref{fig:NR-percentages} shows the percentage of users that is being roamed to another MNO in case of national roaming. This figure shows that under national roaming,  user association changes significantly and at most half of the users of an MNO will connect to that MNO, while the other users connect to the BSs of another MNO. For \Vodafone, this percentage is even lower: only 17.9 $\%$ of their users connect to the BSs of their own MNO. These results are in line with the results shown in Fig.~\ref{fig:FDPFSP}: since \Vodafone provides less coverage to their users, they benefit most from national roaming and therefore many users will use the network of \KPN and \TMobile.}

\begin{figure}
    \centering
    \includegraphics[width = 0.3\textwidth]{Figures/Percentages_to_MNO_Resilience paper.png}
    \caption{Percentage of users in Enschede being served
by each MNO. An arrow shows the percentage of users
of an MNO being roamed to another MNO.}
    \label{fig:NR-percentages}
\end{figure}



%Since a province is a large area with diverse cells and population distribution, it is challenging to investigate causes of these observations in more detail. Therefore, we also analyze the FDP and FSP at the municipality level. For this analysis, we run simulations on province-level and then consider the BSs, users, and performance measures per municipality. Fig.~\ref{fig:FDPFSP_municipalities} depicts the FDP and FSP for 10 Dutch municipalities whose average urbanity level, area, and number of BSs and users per MNO are listed in Table\,\ref{tab:municipality_province_statistics}. While our previous observations also hold here, Fig.~\ref{sfig:FSP_cities} illustrates a more significant difference among MNOs in a municipality. This difference might emerge due to various reasons such as the difference in the number of BSs deployed or the number of users. 
%
% In contrast to our previous conclusion, we now observe negative $\Delta$FSP 
% for \TMobile and \Vodafone in Fig.\ref{sfig:city_gains}. Our further investigation reveals that these are rare cases occurring in very small cities with only few BSs.  \lotte{explain negative FSP}

%Moreover, while \TMobile is almost always the best performer in both metrics, \Vodafone and \KPN might be following \KPN in terms of FSP in different cities, e.g., \Vodafone in Enschede and Amsterdam whereas \KPN in the rest of the municipalities.




%

% Next, to observe the trends for cities of different sizes, let us focus on two municipalities: Amsterdam and Enschede, which reflect a large and a middle-sized municipality, respectively. 
% Fig.~\ref{sfig:SNR_ecdf_Amsterdam} shows the SINR distribution for all operators and under national roaming in Amsterdam. For practical purposes, we subdivided each given area in squares of $50$m$\times50$m and calculated the SINR at the center of each of these squares. For \KPN, $3.3\%$ of the area has an SINR-value below 5\,dB. For \TMobile and \Vodafone and national roaming, this is $2.9\%$, $8.6\%$ and $1.8\%$, respectively. Therefore, for Amsterdam, we observe that a small but non-negligible fraction around $3{-}9\%$ may be under SINR outage, e.g., when $\gamma^{\text{min}}=5$\,dB. We see that these values correspond to the FDP percentages in Fig.~\ref{sfig:FDP_cities}.
% For the municipality of Enschede (Fig.~\ref{sfig:SNR_ecdf_Enschede}), a middle-sized municipality, the observed FDP values are almost the same: $3.2\%, 2.8\%, 8.4\%$ and $1.6\%$ of the area has an SINR-value below 5\,dB for \KPN, \TMobile, \Vodafone and national roaming, respectively. 
% When looking at the shape of the curves in Figs.~\ref{sfig:SNR_ecdf_Amsterdam} and \ref{sfig:SNR_ecdf_Enschede}, we observe only a slight difference for \Vodafone and national roaming, where the curves for Amsterdam and Enschede do not behave the same. For \Vodafone, this difference is related to the density of BSs in both municipalities. Since Enschede has a smaller area, there will be less BSs and therefore \Vodafone cannot provide as high coverage as it could in Amsterdam, where there are more BSs. However, in general, the average SINR in Enschede is higher than the SINR in Amsterdam, especially for national roaming.


% \begin{figure*}[thb]
%     \centering
%     \subcaptionbox{SINR distribution in Amsterdam\label{sfig:SNR_ecdf_Amsterdam}}{\includegraphics[width=.47\textwidth]{Figures/sinr_distributionAmsterdamall_MNOs2150.pdf}}\hfill
%     \subcaptionbox{SINR distribution in Enschede\label{sfig:SNR_ecdf_Enschede}}{\includegraphics[width=.47\textwidth]{Figures/sinr_distributionEnschedeall_MNOs2150.pdf}}
%     \caption{SINR distribution of all MNOs and national roaming in Amsterdam and Enschede. The gray dotted line denotes the threshold SINR $\gamma^\text{min} = 5$dB. }
%     \label{fig:capacity_ecdf}
% \end{figure*}

\begin{tcolorbox}[title=\textbf{Takeaway},colback=gray!20,colframe=white,arc=3mm,boxsep=3mm]
 Our analysis shows that FDP and FSP vary across MNOs and geographic regions. National roaming can consistently offer benefits; up to 13\% improvement in FDP and up to 55\% in FSP. However, the observed benefits vary across MNOs, technologies and regions. Thus, for internet equity, {national roaming can be a solution in those regions not meeting a desired level of FDP and FSP to achieve a certain target level.
Moreover, the simulations show that only sharing a certain technology or in a certain area results in better FDP and FSP, although amount of resources (available spectrum or number of BSs) in this case is the most important factor: sharing more resources generally results in better FDP and FSP.} 
Similarly, MNOs can consider these areas for their own network expansion with newer technologies, including mid-band 5G frequency usage for enhancing FDP and high-band 5G frequencies for enhancing FSP. 
\end{tcolorbox}

% \section{Model assumptions}
% \textit{\begin{itemize}
%     \item There are BSs at height 0 m. However, in the 3GPP RMa NLOS model we divide by the BS height - I now divide by max(1, $h_{BS}$).
% \end{itemize}}

\section{Resilience under failures} \label{sec:perf-failures}
Now, we investigate how failures might affect each MNO in terms of FDP and FSP and how national roaming could help in these cases.  
%
In case of an isolated failure, a cell tower might fail due to software errors~(e.g., misconfiguration or malicious attacks) or hardware errors~(e.g., power loss) independent of the other towers. Also, this type of failure represents the case where MNOs conduct regular maintenance on their network, during which some BSs become out-of-service. 
%
Second, correlated regional failures represent failures in a spatial locality due to certain events, e.g., a thunderstorm in a smaller region or an earthquake or flood affecting a larger region. Failures on the backhaul transport network can also be considered in this category, as such failures affect multiple BSs in a certain region simultaneously~\cite{yanPredictiveImpact,vass2021probabilistic}. In this case, BSs located in the same region will be affected similarly. 
%
For the isolated failures, we test a scenario in which a fraction $p_{\text{iso}}$ of the BSs fails. In the case of a correlated regional failure, all BSs within a circle of radius $r_{\text{fail}}$ meters of the center fail, where we assume the center is the centroid of the region. 
%


% Moreover, a sudden increase of user activity, for instance due to a festival, affects the performance of the network as well. We model this case as a $p_{\text{pop}}$ percent increase of user population in the entire region. 
%
% \lotte{REMOVE? } \suzan{Yes!} Lastly, we investigate the importance of a single BS using the importance metric introduced in \eqref{eq:delta_failure}. To calculate this metric for every BS, we compute the FSP and FDP under a single BS failure for every BS in the municipality. The goal of this analysis is to identify the potential weak points in the network so that MNOs can take proactively actions to avoid the failures in these BSs, e.g., improving power resources against power outages. 

We conduct simulations for these scenarios on the municipality level, each with 100 independent runs for statistical significance. As municipality, we choose Enschede since it is a middle-sized municipality with both urban and rural areas. 
%Moreover, the user population in Enschede will be similar to the address density, which is not the case in municipalities such as Amsterdam, where it is expected that the number of mobile data users and residents are different due to e.g., tourism. 
However, the general results for Enschede are similar to every other municipality and can be found in  \cite{interface}.\footnote{\newInfo{The impact of failures for other cities and provinces can be found on our interactive resilience map of the Netherlands \cite{interface}.}}

\textbf{Isolated failures:} Fig.~\ref{fig:random_failure_nationalroaming} shows each MNO's performance in Enschede in terms of FDP and FSP under isolated failures, where every BS fails independently with probability $p_{\text{iso}}$. Note that $p_{\text{iso}}=0$ corresponds to a scenario without failures. Comparing the performance with this baseline scenario, 
as observed in earlier studies such as \cite{yanPredictiveImpact}, we infer that individual failures do not have a significant impact on the end users due to the inherent signal coverage redundancy in the network. 
However, contradicting the intuitions, Fig.~\ref{sfig:random_failure_NR_FDP} shows that higher $p_{\text{iso}}$ might result in lower FDP.
For instance,  for $p_{\text{iso}}=0.25$, FDP is lower for \KPN and \TMobile compared to the maintained FDP for $p_{\text{iso}}=0$.
%
A closer investigation shows that this is due to a decrease in the interference in the system with the decrease in the number of BSs. For \KPN, the difference between the received SINR and the SNR is $12$dB in a scenario without failures while it is only $9$dB for $p_{\text{iso}} = 0.25$. In other words, the interference decreases with failing BSs resulting in higher SINR on the average leading to lower FDP. However, interference management plays a key role in maintaining a high signal quality and consequently high capacity. Our observations are based on the assumption that MNOs implement interference management schemes and the closest three co-channel BSs do not interfere with each other. However, under other assumptions or a more advanced frequency re-use scheme, these results could be different.
%
%When $p_{\text{iso}}=0.5$, simulations similar to the one in Fig.~\ref{sfig:SNR_ecdf_Enschede} show that the percentage of area where the signal is below $5$dB is on average $1.8\%$, $0.53\%$, $17\%$ and $1.8\%$ for the three MNOs and national roaming, respectively. This implies that even for a failure percentage of $50\%$, almost the entire region is under coverage under national roaming and for users that are subscribed to \KPN or \TMobile. These observations match with the conclusions from Fig.~\ref{sfig:random_failure_NR_FDP}. Thus, these considered MNOs have sufficient redundancy in terms of BSs to account for large number of failures and users can have still access to communications services, which is paramount in the aftermath of extreme events.
%
When it comes to FSP, Fig.~\ref{sfig:random_failure_NR_FSP} suggests that users experience service quality degradation more drastically if MNOs do not implement infrastructure sharing. Failures up to $10\%$ of the BSs do not affect the networks significantly, but for higher values of $p_{\text{iso}}$ the surviving BSs become overloaded~(i.e., has to serve an increased number of users) which causes degradation in user satisfaction represented by lower FSP. 
%
Note that the decrease in FSP can be mitigated by dynamic frequency allocation schemes which re-allocate the frequency resources of the failing BSs to the active ones. 
%
Comparing the benefit of infrastructure sharing under normal operation~($p_{\text{iso}}=0$) against that of under failures~($p_{\text{iso}}>0$) by accounting for both FDP and FSP, we can conclude that sharing 
leads to better performance under failures. The networks of \KPN and \TMobile in particular are sufficiently redundant to still ensure coverage under failures. However, to also ensure satisfaction, network sharing is paramount.


% \textcolor{red}{Could we have models from Fernando's paper on modelling failures? \url{https://pure.tudelft.nl/ws/portalfiles/portal/96545736/m93889_vass.pdf}}

\begin{figure*}[htb]
    \centering
    \subcaptionbox{FDP\label{sfig:random_failure_NR_FDP}}{\includegraphics[width=.45\textwidth]{Figures/random_fdp.pdf}}\hfill
    \subcaptionbox{FSP \label{sfig:random_failure_NR_FSP}}{\includegraphics[width=.45\textwidth]{Figures/random_fsp.pdf}}\hfill
    \caption{FDP and FSP under isolated failures in Enschede for different MNOs, where each BS fails with probability $p_{\text{iso}}$.    \label{fig:random_failure_nationalroaming} }
    % \textcolor{blue}{It deserves a convincing discussion on why the failures improve FDP for MNO1 and MNO2. If the main argument is interference, this should be shown with change in the interference distribution.} }
    % \syllas{I think that these weird results related to interference might have to do with the consideration that all BSs are operating at ``full power'' (90\% of EIRP) even when it is not necessary to meet the users rate requirement (is it really the case?), but I would expect it to be even more problematic with national roaming due to the proximity of the BSs. } } 
\end{figure*}

\begin{figure*}[htb]
    \centering
    \subcaptionbox{FDP\label{sfig:correlated_failure_NR_FDP}}{\includegraphics[width=.45\textwidth]{Figures/disaster_fdp.pdf}}\hfill
    \subcaptionbox{FSP \label{sfig:correlated_failure_NR_FSP}}{\includegraphics[width=.45\textwidth]{Figures/disaster_fsp.pdf}}\hfill
    \caption{FDP and FSP under correlated failures in Enschede, where all BSs within  $r_{\text{fail}}$ meters of the center fail. \label{fig:correlated_failure_nationalroaming}}
    % \textcolor{blue}{Not sure if I can explain these figures clearly. When radius of failure is large, FDP is lower for MNO-1. Even lower than national roaming. }} 
    
\end{figure*}

\textbf{Correlated failures:} Fig.~\ref{fig:correlated_failure_nationalroaming} plots the FDP and FSP with increasing radius of correlated failures. In every case, we simulate a failure in the center of the municipality and let all BSs within radius $r_\text{fail}$ m of the center fail. If $r_\text{fail} = 500$m, on average $1\%$ of the BSs in the region fail. For $r_\text{fail} = 100, 2500$ and $5000$m, this is respectively $9\%, 38\%$ and $65\%$ of the BSs.

Similar to the isolated failures in Fig.~\ref{fig:random_failure_nationalroaming}, Fig.~\ref{fig:correlated_failure_nationalroaming} suggests that the FDP and FSP are not affected for small regions of failure under correlated failures. However, for larger radii, we notice that national roaming does not result in the highest FSP and lowest FDP anymore~(e.g., when $r_{\text{fail}}=2500$ m), as \KPN performs better in terms of FDP and \TMobile in terms of FSP. 
We attribute this lower FSP to a higher number of users served by the remaining surviving BSs. Under national roaming, three times as many users are in the center of a region (the city center) compared to no national roaming. Moreover, due to the non-uniform deployment of BSs, the number of BSs that fail is relatively large compared to a single-MNO scenario. Hence, a disaster in this region has more impact when all users share the network compared to when every MNO uses its own network, as BSs on the border of the disaster region become more congested. Comparing Fig.~\ref{sfig:correlated_failure_NR_FSP} and Fig.~\ref{sfig:random_failure_NR_FSP}, correlated failures  causes a significantly lower satisfaction compared to isolated failures, e.g., for $r_\text{fail} = 2500$m, around $38\%$ of the BSs fail, but the FSP is lower than the FSP for $p_\text{iso} = 0.5$.




\begin{tcolorbox}[title=\textbf{Takeaway},colback=gray!20,colframe=white,arc=3mm,boxsep=3mm]
Our analysis shows that isolated failures do not lead to any significant FDP decrease as the MNOs have enough redundancy in terms of the BSs covering an area: even if 50$\%$ of the BSs in a region fails, most users still maintain the required minimum signal level for connectivity. On the contrary, the FSP  drastically decreases, as BSs become more congested and the effective user bandwidth decreases due to the increase in the number of users served by the surviving BSs. Correlated failures lead to a more significant impact compared to isolated failures, i.e., increase in FDP and decrease in FSP. However, in most cases, numerical analysis shows that national roaming has the potential to improve resilience. 
\end{tcolorbox}



% \begin{figure*}[thb]
%     \centering
%     \subcaptionbox{FDP\label{sfig:correlated_failure_NR_FDP}}{\includegraphics[width=.5\textwidth]{Figures/national_roamingall_MNOs21disaster50005FDPmunicipalities.png}}\hfill
%     \subcaptionbox{FSP \label{sfig:correlated_failure_NR_FSP}}{\includegraphics[width=.5\textwidth]{Figures/national_roamingall_MNOs21disaster50005FSPmunicipalities.png}}\hfill
%     \caption{FDP and FSP under correlated failures in Enschede for different MNOs, where all BSs within radius $r_{\text{fail}}$ meters of the center fail.} 
%     \label{fig:correlated_failure_nationalroaming}
% \end{figure*}



% \begin{figure*}[thb]
%     \centering
%     \subcaptionbox{FDP\label{sfig:FDP_cities_user_increaseKPN}}{\includegraphics[width=.5\textwidth]{Figures/KPN20.33user_increase2005FDPmunicipalities.png}}\hfill
%     \subcaptionbox{FSP \label{sfig:FSP_cities_user_increaseKPN}}{\includegraphics[width=.5\textwidth]{Figures/KPN20.33user_increase2005FSPmunicipalities.png}}\hfill
%     \caption{FDP and FSP with $p_{\text{pop}}$ percent user increase for \KPN.} 
%     \label{fig:FDPFSP_user_increase_KPN}
% \end{figure*}

%\subsection
% \textbf{User increase:} \textcolor{blue}{SB: this explanation is not aligned with the figure. why would fdp change?} Fig.~\ref{fig:user_increase_nationalroaming} shows the FDP and FSP under an increased number of users in Enschede. We can see that in general, the FDP remains similar but the FSP level decreases for increasing number of users, as the resources are then divided among more users. In agreement with earlier observations, national roaming has a superior performance, although \TMobile has a similar performance in terms of FSP.

% {up to a certain extent, when the user increase is $200\%$. However, while the FSP for \TMobile for $200\%$ is higher compared to national roaming, the FDP for \TMobile is also higher. This means that \TMobile will serve less users but with higher satisfaction, while national roaming focuses on serving more uses. \lotte{is this possible?}

% \begin{figure*}[thb]
%     \centering
%     \subcaptionbox{FDP\label{sfig:user_increase_NR_FDP}}{\includegraphics[width=.5\textwidth]{Figures/national_roamingall_MNOs21user_increase2005FDPmunicipalities.png}}\hfill
%     \subcaptionbox{FSP \label{sfig:user_increase_NR_FSP}}{\includegraphics[width=.5\textwidth]{Figures/national_roamingall_MNOs21user_increase2005FSPmunicipalities.png}}\hfill
%     \caption{FDP and FSP under user increase in Enschede for different MNOs.} 
%     \label{fig:user_increase_nationalroaming}
% \end{figure*}
 
% \textbf{{BS importance}:} Fig.~\ref{fig:delta_FSP_FDP} shows $\Delta_j^{\text{fsp}}$ and $\Delta_j^{\text{fdp}}$ for each BS  in Enschede. 
% In general, failure of a single BS will result in a higher FDP~(negative $\Delta^{\text{fdp}}$) and a lower FSP (positive $\Delta^{\text{fsp}}$). 
% In some cases, however, we might observe different trends. For instance, the removal of a single BS of \KPN results in a slightly higher satisfaction of the users~(Fig.~\ref{sfig:FSP_improvement}), although this is at the expense of more disconnected users~(Fig.~\ref{sfig:FDP_improvement}).  
% %
%  We speculate that this increase in FSP for \KPN might be due to its uniform BS deployment in Enschede compared to the other MNOs. 
%  As Fig.~\ref{fig:random_failure_nationalroaming} shows, there is redundancy in the number of BSs. Thus, removing a single BS will not drastically change the network performance and might even improve it due to less interference. In combination with the uniform deployment of \KPN, this implies that in general users of \KPN are closer to a BS (so higher SNR) and will therefore have a high satisfaction. However, due to this uniform deployment, a BS failure in a densely-populated area results in more disconnected users compared to the other MNOs, where more BSs are deployed in densely populated areas. Hence, the FDP for \KPN is slightly higher on average.
%  This shows that resilient networks in terms of coverage or capacity do not necessarily look similar. 
% % 
% Fig.~\ref{sfig:FSP_improvement} shows that national roaming will result in the highest decrease in FSP. A reason for this is that when one cell tower fails, under national roaming, more BSs will fail. However, since the FSP is higher with national roaming compared to a single provider, the resulting FSP will still be higher.

% \begin{figure*}[thb]
%     \centering
%     \subcaptionbox{FDP\label{sfig:user_increase_NR_FDP}}{\includegraphics[width=.5\textwidth]{Figures/user_increase_fdp.pdf}}\hfill
%     \subcaptionbox{FSP \label{sfig:user_increase_NR_FSP}}{\includegraphics[width=.5\textwidth]{Figures/user_increase_fsp.pdf}}\hfill
%     \caption{FDP and FSP under increase in number of users in Enschede for different MNOs.} 
%     \label{fig:user_increase_nationalroaming}
% \end{figure*}

% \lotte{We do not say much about the user increase plots. Maybe leave them out?}\textcolor{red}{Clara: Yes then we can also tell rhe referees that we reduced the number of plots.}
% \begin{figure}
%     \centering
%     \includegraphics[width = 0.49\textwidth]{Figures/delta_fsp_fdp_Enschede.png}
%     \caption{$\Delta_j^{\text{fsp}}$ and $\Delta_j^{\text{fdp}}$ for each BS$_j$ in Enschede}
%     \label{fig:delta_failure_Enschede}
% \end{figure}

% \begin{figure*}[thb]
%     \centering
%     \subcaptionbox{FDP \label{sfig:FDP_improvement}}{\includegraphics[width=.5\textwidth]{Figures/FDP_improvement.png}}\hfill
%     \subcaptionbox{FSP \label{sfig:FSP_improvement}}{\includegraphics[width=.5\textwidth]{Figures/FSP_improvement.png}}\hfill
%     \caption{$\Delta_j^{\text{fdp}}$ and $\Delta_j^{\text{fsp}}$ in Enschede for the three providers and national roaming. \lotte{Also leave out this figure? + text}} 
%     \label{fig:delta_FSP_FDP}
% \end{figure*}



==> 6.discussion.tex <==
\section{Discussion and Limitations}\label{sec:discussion}

To have a realistic representation of the current cellular networks, we  used publicly available datasets. Hence, we are limited with the limitations of the data. While national bodies are more reliable source of information on the MNOs' infrastructures compared to crowdsourced datasets, the datasets might be incomplete, e.g., mobile coverage points to offer rural area coverage not being recorded in the dataset. 
% 
Another caveat is that we had to make some assumptions and simplifications about the operation of these networks. For instance, we have not considered thoroughly the interference management and coordination approaches which are typically applied by the network operators. In real operation, there are many knobs (e.g., from interference cancellation to power adaptation) that would change the SINR and hence the channel capacity and consequently the achieved satisfaction of the user. 
%
Hence, our results should be interpreted with these shortcomings in mind. 
%



We used the 3GPP path loss models to model the signal loss in different areas. However, our models only use an independent path loss probability for every link. Path loss by buildings or blockers is not   independently distributed for every link and this  affects the signal propagation. 
Nevertheless, we believe that our analysis maintains a good balance between realism and tractability. %Studying the effect of blockers on small-scale areas is an interesting direction for further research, for example by using available building and vegetation data.   

To mitigate the time complexity while assessing the quality and resilience in a certain area such as a province or municipality, we considered each area as an isolated network. More particularly, the users, the BSs that are within the borders of that particular region and the BSs within 2000 meters of this border are considered. Consequently, users at the areas close to the borders of these regions can connect to the BSs in the neighboring regions. Since we have not considered the users of that neighboring region that would be connecting to those BSs, our performance results might be overestimating the reality. 

\newInfo{Due to the limited availability of data about each MNO, we have assumed an equal user distribution among MNOs, which may be unrealistic. We chose not to use market reports that indicate the users shares per MNO, as it is still not public how mobile virtual operators use the physical operators' network.} 
Moreover, we have assumed that the number of users in a certain region is proportional to the population of that region. However, reality could differ from this distribution as the number of cellular users in an area depends also on business or social activities of that region, e.g., a hotspot business area attracting many people from other regions. Moreover, our analysis considered only a throughput and coverage perspective. For 5G networks, there are various new applications whose performance is assessed by other metrics such as packet loss or latency. To have a more rigorous understanding of the national cellular network performance and to identify the regions that should be prioritized in service enhancement, national agencies~(e.g., {\color{black}\textit{Rijksinspectie Digitale Infrastructuur}} in the Netherlands or Ofcom in the UK) can maintain maps of cellular network availability and speed performance similar to the maps for broadband connectivity~\cite{NTIA_broadband_map}.

% FCC challenge https://cands.cc.gatech.edu/blog/what-does-it-take-fcc-challenge/ and broadband map 

Finally, more knowledge on the temporal dynamics of a cellular network, e.g., number of served users during peak and off-peak hours, and application requirements can 
%it would be interesting to obtain more data on the user's side. What is the rate requirement of an average user? And what is the fraction of connected users during peak hours, or during less congested hours of the day in terms of internet usage? 
%These additional data would 
provide a more realistic performance assessment of the networks. For example, nation-wide crowd-sensing campaigns such as \cite{cellmapper} could help with collecting this data by reflecting the users' experience on different geographies including rural areas and with all cellular operators in the proximity of the user. These on-site measurements can be an input to both the national coverage maps and to MNOs for their network planning and assessing the potential benefits of infrastructure sharing. \newInfo{To show the benefits of network sharing, one could also investigate how much the number of resources in a shared network can be decreased compared to the situation nowadays. As MNOs typically over-provision their network to ensure user satisfaction even in case of a failure, network sharing can help in less over-provisioning and therefore lower energy usage.}

{To measure the full resilience of a cellular network under correlated failures caused by a disaster such as an earthquake or a flood, one cannot forget the backbone. We did not model the backbone and therefore our results only show a best-case scenario: failures in the backbone network only degrades the performance, e.g., increasing FDP and decreasing FSP. Investigating and quantifying the effect of such correlated failures is therefore an interesting topic for further research. } 

%Similarly, the resilience metrics provided here could also be adapted to different types of failures such as \cite{vass2021probabilistic}. 

% maybe mention different modes of Mobile Network sharing as investigated in \cite{panchal2013mobile}



==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> table_BS_data.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{l|ccccc|ccccc}
\multicolumn{1}{c|}{\textit{}}         & \multicolumn{5}{c|}{\textit{# BS (min - max)  per km$^2$}}           & \multicolumn{5}{c}{\textit{Average #BS per km$^2$}}                                                                                      \\
\multicolumn{1}{c|}{\textit{Urbanity}} & \textit{1}   & \textit{2}  & \textit{3}  & \textit{4}  & \textit{5}  & \textit{1}                & \textit{2}               & \textit{3}                & \textit{4}               & \textit{5}                 \\ \hline
\textbf{Netherlands}                   & \textbf{129} & \textbf{42} & \textbf{62} & \textbf{21} & \textbf{22} & \textbf{17}               & \textbf{7}               & \textbf{4}                & \textbf{2}               & \textbf{0.7}               \\ \hline
Overijssel                             & 37           & 42          & 21          & 10          & 9           & {\color[HTML]{FE0000} 15} & {\color[HTML]{FE0000} 6} & {\color[HTML]{333333} 4}  & {\color[HTML]{333333} 2} & {\color[HTML]{009901} 0.6} \\
Gelderland                             & 41           & 19          & 17          & 15          & 7           & {\color[HTML]{FE0000} 14} & {\color[HTML]{333333} 7} & {\color[HTML]{333333} 4}  & {\color[HTML]{333333} 2} & {\color[HTML]{333333} 0.7} \\
Noord-Holland                          & 76           & 19          & \textbf{62} & 12          & \textbf{22} & {\color[HTML]{009901} 18} & {\color[HTML]{FE0000} 6} & {\color[HTML]{333333} 4}  & {\color[HTML]{333333} 2} & {\color[HTML]{009901} 1}   \\
Zuid-Holland                           & \textbf{129} & 40          & 19          & 7           & 9           & {\color[HTML]{009901} 19} & {\color[HTML]{333333} 7} & {\color[HTML]{333333} 4}  & {\color[HTML]{333333} 2} & {\color[HTML]{009901} 1}   \\
Groningen                              & 5 - 36       & 3 - 9       & 12          & 0.4 - 6     & 8           & {\color[HTML]{FE0000} 15} & {\color[HTML]{FE0000} 6} & {\color[HTML]{FE0000} 3}  & {\color[HTML]{333333} 2} & {\color[HTML]{FE0000} 0.4} \\
Utrecht                                & 73           & 19          & 22          & \textbf{21} & 2           & {\color[HTML]{009901} 18} & {\color[HTML]{FE0000} 6} & {\color[HTML]{009901} 5}  & {\color[HTML]{009901} 3} & {\color[HTML]{333333} 0.7} \\
Limburg                                & 8 - 33       & 20          & 1 - 12      & 17          & 7           & {\color[HTML]{333333} 17} & {\color[HTML]{009901} 8} & {\color[HTML]{009901} 5}  & {\color[HTML]{333333} 2} & {\color[HTML]{009901} 1}   \\
Zeeland                                & 5 - 7        & 13          & 14          & 6           & 9           & {\color[HTML]{FE0000} 6}  & {\color[HTML]{333333} 7} & {\color[HTML]{FE0000} 3}  & {\color[HTML]{FE0000} 1} & {\color[HTML]{333333} 0.7} \\
Noord-Brabant                          & 36           & 16          & 25          & 12          & 19          & {\color[HTML]{FE0000} 14} & {\color[HTML]{FE0000} 6} & {\color[HTML]{333333} 4}  & {\color[HTML]{333333} 2} & {\color[HTML]{009901} 1}   \\ \hline
Enschede                               & 37           & 2 - 10      & 3           & 2 - 3       & 2           & {\color[HTML]{FE0000} 16} & {\color[HTML]{FE0000} 5} & {\color[HTML]{FE0000} 2}  & {\color[HTML]{333333} 2} & {\color[HTML]{009901} 0.8} \\
Amsterdam                              & 76           & 5 - 15      & \textbf{62} & /           & 6           & {\color[HTML]{009901} 24} & {\color[HTML]{009901} 8} & {\color[HTML]{009901} 31} & /                        & {\color[HTML]{009901} 2}   \\
Rotterdam                              & 7 - 124      & 2 - 19      & 15          & 5           & 2 - 9       & {\color[HTML]{009901} 26} & {\color[HTML]{009901} 8} & {\color[HTML]{009901} 5}  & {\color[HTML]{009901} 3} & {\color[HTML]{009901} 5}   \\
Zwolle                                 & 5 - 24       & 3 - 7       & 2 - 21      & 7           & 2           & {\color[HTML]{FE0000} 14} & {\color[HTML]{FE0000} 5} & {\color[HTML]{009901} 9}  & {\color[HTML]{333333} 2} & {\color[HTML]{009901} 1}   \\
Assen                                  & /            & 3-8         & 3-4         & 2-3         & 2           & /                         & {\color[HTML]{FE0000} 6} & {\color[HTML]{333333} 4}  & {\color[HTML]{009901} 3} & {\color[HTML]{333333} 0.7}
\end{tabular}%
}
\caption{Minimum, maximum and average number of BSs per province/municipality}
\label{tab:BSs_data}
\end{table}
